GAIT: A Geometric Approach to Information Theory

We advocate the use of a notion of entropy that reflects the relative abundances of the symbols in an alphabet, as well as the similarities between them. This concept was originally introduced in theoretical ecology to study the diversity of ecosystems. Based on this notion of entropy, we introduce geometry-aware counterparts for several concepts and theorems in information theory. Notably, our proposed divergence exhibits performance on par with state-of-the-art methods based on the Wasserstein distance, but enjoys a closed-form expression that can be computed efficiently. We demonstrate the versatility of our method via experiments on a broad range of domains: training generative models, computing image barycenters, approximating empirical measures and counting modes.

==> imgs/mais_toy_entropy.tex <==
\begin{figure}[h]
	\begin{minipage}{.28\textwidth}
		\centering
		\vspace{-4mm}
		\includegraphics[trim=0 0 0 0, clip, width=0.92\textwidth]{imgs/ent_2d.png}
		\captionof{figure}{$\mathbb{H}^\mK_1$ interpolates towards Shannon's entropy.}
		\label{fig:ent_2d}
	\end{minipage}
	\hspace{6mm}
	\begin{minipage}{.3\textwidth}
		\vspace{1mm}
		\hspace{1mm}
		\begin{tikzpicture}[<->,>=stealth',shorten >=1pt,auto,node distance=2cm, scale=0.85, every node/.style={scale=0.85}, thick, main node/.style={circle, draw}]
		
		\node[main node] (a) {A};
		\node[main node] (b) [below of=a] {B};
		\node[main node] (c) [above right=0.5cm and 2.1cm of b] {C};
		
		\path
		(a) edge [loop left] node {1} (a)
		edge node [left] {0.7} (b)
		edge node {0.1} (c)
		(b) edge [loop left] node {1} (b)
		(c) edge [loop above] node {1} (c)
		edge node {0.1} (b);
		\end{tikzpicture}
		\vspace{2mm}
		\captionof{figure}{A 3-point space with two highly similar elements.}
		\label{fig:3pt_space}
	\end{minipage}
	\hfill
	\begin{minipage}{.3\textwidth}
		\centering
		\vspace{-1mm}
		\includegraphics[width=0.93\textwidth]{imgs/toy_heatmap.png}
		\captionof{figure}{Entropy heatmap of the space in Fig. \ref{fig:3pt_space}.}
		\label{fig:toy_heatmap}
	\end{minipage}
\end{figure}
